Time Series Copulas for Heteroskedastic Data

We propose parametric copulas that capture serial dependence in stationary heteroskedastic time series. We develop our copula for first order Markov series, and extend it to higher orders and multivariate series. We derive the copula of a volatility proxy, based on which we propose new measures of volatility dependence, including co-movement and spillover in multivariate series. In general, these depend upon the marginal distributions of the series. Using exchange rate returns, we show that the resulting copula models can capture their marginal distributions more accurately than univariate and multivariate GARCH models, and produce more accurate value at risk forecasts.

==> defs_letter.tex <==
\setlength{\topmargin}{-0.75in}
\setlength{\textheight}{9.5in}
\setlength{\oddsidemargin}{0pt}
%\textwidth 440pt 
\setlength{\textwidth}{6.5in}%width for US letterhead paper 
\parskip 0pt
\newcounter{num}
\newcommand{\utilde}[1]{\mathrel{\mathop{#1}\limits_{\displaystyle \widetilde{}}}}
%\def\baselinestretch{1.22}
\def\theequation{\thesection.\arabic{equation}}  
\def\abstract{\if@twocolumn
\section*{Abstract}
\else \normalsize 
\begin{center}
{\bf Summary\vspace{-.5em}\vspace{0pt}} 
\end{center}
\quotation 
\fi}
\def\endabstract{\if@twocolumn\else\endquotation\fi}
\newcommand{\bfy}{\mbox{{\bf y}}}
\newcommand{\bfw}{\mbox{\boldmath $w$}}
\newcommand{\bfs}{\mbox{\boldmath $s$}}
\newcommand{\bfg}{\mbox{\boldmath $g$}}
\newcommand{\bfu}{\mbox{\boldmath $u$}}
\newcommand{\bfv}{\mbox{\boldmath $v$}}
\newcommand{\bfx}{\mbox{\boldmath $x$}}
\newcommand{\bfzero}{\mbox{{\bf 0}}}
\newcommand{\bfalpha}{\mbox{\boldmath $\alpha$}}
\newcommand{\bfmu}{\mbox{\boldmath $\mu$}}
\newcommand{\bff}{\mbox{{\bf f}}}
\newcommand{\bfb}{\mbox{{\bf b}}}
\newcommand{\bfone}{\mbox{{\bf 1}}}
\newcommand{\bfZ}{\mbox{\boldmath $Z$}}
\newcommand{\bfe}{\mbox{{\bf e}}}
\newcommand{\bfr}{\mbox{{\bf r}}}
\newcommand{\bfz}{\mbox{{\bf z}}}
\newcommand{\told}{\mbox{{\tiny old}}}
\newcommand{\tnew}{\mbox{{\tiny new}}}
\newcommand{\gammanew}{\mbox{$\gamma^{\tnew}$}}
\newcommand{\gammajnew}{\mbox{$\gamma^{\tnew}_j$}}
\newcommand{\gammaold}{\mbox{$\gamma^{\told}$}}
\newcommand{\gammajold}{\mbox{$\gamma^{\told}_j$}}
\newcommand{\zetan}{\mbox{$\zeta^{\tnew}$}}
\newcommand{\zetao}{\mbox{$\zeta^{\told}$}}
\newcommand{\phin}{\mbox{$\phi^{\tnew}$}}
\newcommand{\phio}{\mbox{$\phi^{\told}$}}
\newcommand{\phitn}{\mbox{$\tilde \phi^{\tnew}$}}
\newcommand{\phito}{\mbox{$\tilde \phi^{\told}$}}
\newcommand{\bfJ}{\mbox{\boldmath $J$}}
\newcommand{\bfpsi}{\mbox{\boldmath $\psi$}}
\newcommand{\bfepsilon}{\mbox{\boldmath $\epsilon$}}
\newcommand{\bfgamma}{\mbox{\boldmath $\gamma$}}
\newcommand{\bfbeta}{\mbox{\boldmath $\beta$}}
\newcommand{\bfomega}{\mbox{\boldmath $\omega$}}
\newcommand{\bfkappa}{\mbox{\boldmath $\kappa$}}
\newcommand{\bftheta}{\mbox{\boldmath $\theta$}}
\newcommand{\half}{\mathop{\frac{1}{2}}}
\newcommand{\var}{\mathop{\rm var}} 
\newcommand{\Exp}{\mathop{\rm E}}
\newcommand{\cov}{\mathop{\rm cov}}
\newcommand{\corr}{\mathop{\rm corr}}
\newcommand{\rank}{\mathop{\rm rank}}
\newcommand{\load}{\mbox{LOAD}}
\newcommand{\temp}{\mbox{TEMP}}
\newcommand{\hmd}{\mbox{HMD}}
\newcommand{\toy}{\mbox{TOY}}
\newcommand{\dum}{\mbox{DUM}}
\newcommand{\rowspace}{\mathop{\rm row~space}}
\makeatletter
\@addtoreset{equation}{section}
\makeatother
\newtheorem{lemma}{Lemma}[section]
\newtheorem{remark}{Remark}[section]
\newenvironment{Remark}{\begin{remark} \rm}{\end{remark}}
\newcommand{\myappendix}[1]{
%	\renewcommand{\thesection}{{\bf Appendix}~{\bf \Alph{section}}}
%	\section{#1}
	\setcounter{section}{1}
%	\renewcommand{\thesection}{\Alph{section}}} 
        \renewcommand{\thesection}{A\arabic{section}}}

\newcommand{\fah}[1]{
	\vspace{-0.2in}\nopagebreak
	\begin{center}
		{\sf -----#1-----}
	\end{center}\nopagebreak
	\vspace{-0.1in}}

\makeatletter
%% The "\@seccntformat" command is an auxiliary command
%% (see pp. 26f. of 'The LaTeX Companion,' 2nd. ed.)
\def\@seccntformat#1{\@ifundefined{#1@cntformat}%
   {\csname the#1\endcsname\quad}  % default
   {\csname #1@cntformat\endcsname}% enable individual control
}
\let\oldappendix\appendix %% save current definition of \appendix
\renewcommand\appendix{%
    \oldappendix
    \newcommand{\section@cntformat}{\appendixname~\thesection\quad}
}
\makeatother
\usepackage{cleveref} % just for this example



